PuppetAI: A Customizable Platform for Designing Tactile-Rich Affective Robot Interaction

We introduce PuppetAI, a modular soft robot interaction platform. This platform offers a scalable cable-driven actuation system and a customizable, puppet-inspired robot gesture framework, supporting a multitude of interaction gesture robot design formats. The platform comprises a four-layer decoupled software architecture that includes perceptual processing, affective modeling, motion scheduling, and low-level actuation. We also implemented an affective expression loop that connects human input to the robot platform by producing real-time emotional gestural responses to human vocal input. For our own designs, we have worked with nuanced gestures enacted by "soft robots" with enhanced dexterity and "pleasant-to-touch" plush exteriors. By reducing operational complexity and production costs while enhancing customizability, our work creates an adaptable and accessible foundation for future tactile-based expressive robot research. Our goal is to provide a platform that allows researchers to independently construct or refine highly specific gestures and movements performed by social robots.

==> Sections/Challenges_and_Future_Directions.tex <==
\section{Discussions and Future Directions}
\label{sec:challenges and future directions}
Currently, our system employs a ChatGPT-based LLM to trigger predefined action sequences. Future work will explore how to improve the LLM’s ability to interpret verbal and non-verbal human emotional cues and move beyond presets, allowing it to generate dynamic, expressive gestural responses in real-time. We also aim to expand the robot’s expressive abilities through several multimodal upgrades. First, we intend to deploy pneumatic inflation systems beneath the robot’s skin to simulate varied tactile sensations. Second, we plan to incorporate synthetic speech to investigate how vocal tone, style, and the spatial localization of sound influence human empathy and perception. Finally, we will develop larger, life-sized puppets to analyze how physical scale and material properties affect the psychological experience of users interacting with robots.

For hardware improvement, we plan to increase motor density to achieve higher DoFs and more fluid movement while reducing the overall size of the base platform. Future developments will also focus on system-level integration, embedding the control software directly into the hardware platform alongside voice-command interfaces and localized touch-screen controls.
